Communication-Safe Web Programming in TypeScript with Routed Multiparty Session Types

Modern web programming involves coordinating interactions between browser clients and a server. Typically, the interactions in web-based distributed systems are informally described, making it hard to ensure correctness, especially communication safety, i.e. all endpoints progress without type errors or deadlocks, conforming to a specified protocol. We present STScript, a toolchain that generates TypeScript APIs for communication-safe web development over WebSockets, and RouST, a new session type theory that supports multiparty communications with routing mechanisms. STScript provides developers with TypeScript APIs generated from a communication protocol specification based on RouST. The generated APIs build upon TypeScript concurrency practices, complement the event-driven style of programming in full-stack web development, and are compatible with the Node.js runtime for server-side endpoints and the React.js framework for browser-side endpoints. RouST can express multiparty interactions routed via an intermediate participant. It supports peer-to-peer communication between browser-side endpoints by routing communication via the server in a way that avoids excessive serialisation. RouST guarantees communication safety for endpoint web applications written using STScript APIs. We evaluate the expressiveness of STScript for modern web programming using several production-ready case studies deployed as web applications.

==> theory/org_semantics.tex <==
\subsection{Semantics}
We define the labelled transition system (LTS) semantics
over global types
and local types
for \newtheory,
building upon the work of
\citet{2013Automata}.
We show the soundness and completeness of projection
with respect to the LTSs through proving the
\emph{trace equivalence} of
a global type and the collection of local types projected
from the global type.
We then use this result to
conclude that \newtheory provide the same
communication safety guarantees from canonical
MPST theory for well-formed global types,
namely deadlock freedom .

First, we extend the label in the LTS, as shown in
\cref{def:newlts}, to distinguish
the \emph{direct} sending (and reception) of a message
from the sending (and reception) of a message
\emph{via} an intermediate routing endpoint.

\begin{definition}[Labels]
Labels range over $\lbl{l, l', \cdots}$
\[\begin{array}{rlr}
\lbl{l} ::= & & \text{Labels} \\
	\mid & \aout{p}{q}{j} &
		\text{Direct Send} \\
	\mid & \ain{p}{q}{j} &
		\text{Direct Receive} \\
    \rowcolor{ColourShade} \mid & \via{s}{\aout{p}{q}{j}} &
		\text{Routed Send} \\
    \rowcolor{ColourShade}\mid & \via{s}{\ain{p}{q}{j}} &
		\text{Routed Receive} \\
\end{array}\]
\label{def:newlts}
\end{definition}

\begin{itemize}
\item \textbf{Routed Send:}

The label $\via{s}{\aout{p}{q}{j}}$ represents the
\textit{sending} (performed by $\ppt{p}$)
of a message labelled $\lbl{j}$ to $\ppt{q}$ through
the intermediate router $\ppt{s}$.

\item \textbf{Routed Receive:}

The label $\via{s}{\ain{p}{q}{j}}$ represents the
\textit{reception} (initiated by $\ppt{q}$)
of a message labelled $\lbl{j}$
send from $\ppt{p}$ through
the intermediate router $\ppt{s}$.
\end{itemize}

\noindent
Labels represent communication actions, so we refer
to $\lbl{l}$ as labels and actions interchangeably,
as is the case in the literature.

Building upon \cite{2013Automata},
the \emph{subject} of a label is the role
that initiates the action.
Intuitively, the actions for routed send and routed
receive are still initiated by the original sender and
recipient respectively;
we extend the definition
of subjects in \cref{def:newsubj} to reflect this.

\begin{definition}[Subject]
The subject of a LTS label, or $\subj{\lbl{l}}$, is defined as:

\begin{gather*}
\subj{\via{s}{\aout{p}{q}{j}}} =
	\subj{\aout{p}{q}{j}} = \ppt{p} \\
\subj{\via{s}{\ain{p}{q}{j}}} =
	\subj{\ain{p}{q}{j}} = \ppt{q} \\
\end{gather*}

\label{def:newsubj}
\end{definition}

\paragraph{LTS Semantics over Global Types}
The LTS semantics presented in \cite{2013Automata}
models \emph{asynchronous communication},
which is consistent with our proposal.
In order to define LTS over global types for
asynchronous communication, we need to
represent intermediate states (i.e. messages in transit)
within the grammar of global types.
\Citet{2013Automata}
added the construct
$\gtrans{p}{q}{j}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}$
to represent that the message $l_j$ has been
sent by $\ppt p$ but not yet received by $\ppt q$.

We add a similar construct
$\gtransroute{p}{q}{s}{j}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}$
to represent that the message $l_j$ has
been sent from $\ppt{p}$ to the router $\ppt{s}$
\emph{but not yet routed to $\ppt{q}$}.
We extend the projection operator to
support this new construct.

\[
\proj{\gtransroute{p}{q}{s}{j}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}{r} = \begin{cases}
\tbraproxy{p}{s}{\lbl{l_i}\!:\! \proj{G_i}{r}}{\lbl{i \in I}}
	& \text{if } \ppt{r} = \ppt{q} \\
\routertrans{p}{q}{j}{\lbl{l_i}\!:\! \proj{G_i}{r}}{\lbl{i \in I}}
	& \text{if } \ppt{r} = \ppt{s} \\
\proj{G_j}{r}
	& \text{o.w.} \\
\end{cases}
\]

Because the router holds a ``global perspective''
on the routed communication, we also need to
represent the intermediate state (at which the message is
being routed by the router) within the grammar
of \emph{local types}.
We extend the grammar of local types with the construct
$\routertrans{p}{q}{j}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}$
to represent that, from the local perspective of
the router, the message $\lbl{l_j}$
has been received from $\ppt{p}$ \emph{but not yet routed
to $\ppt{q}$}.

Because routed communication is treated differently
from direct send and receive actions, the notion
of asynchrony differs between the two types of communication
too. This definition allows us to extend
the LTS semantics from \cite{2013Automata}
more naturally.

We define the LTS semantics
over global types,
denoted by $\gtreduce{G}{G'}{l}$,
in \cref{fig:newglobal}.
We highlight and explain the new rules.

\begin{figure}[!h]

\begin{prooftree}
\AxiomC{}
\RightLabel{\rulename{Gr1}}
\UnaryInfC{$
\treducelong
	{\gcomm{p}{q}{\lbl{l_i}\!:\! G_i}{i \in I}}
	{\gtrans{p}{q}{j}{\lbl{l_i}\!:\! G_i}{i \in I}}
	{\aout{p}{q}{j}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{}
\RightLabel{\rulename{Gr2}}
\UnaryInfC{$
\gtreducelong
	{\gtrans{p}{q}{j}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}
	{G_j}
	{\ain{p}{q}{j}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$
\gtreduce
	{G[\gtrecur{t}{G} / \gtvar{t}]}
	{G'}
	{l}
$}
\RightLabel{\rulename{Gr3}}
\UnaryInfC{$
\gtreduce
	{\gtrecur{t}{G}}
	{G'}
	{l}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$\forall \lbl{i \in I}. ~ \gtreduce{G_i}{G'_i}{l}$}
\AxiomC{$\subj{\lbl{l}} \notin \{\ppt{p}, \ppt{q}\}$}
\RightLabel{\rulename{Gr4}}
\BinaryInfC{$
\gtreducelong
	{\gcomm{p}{q}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}
	{\gcomm{p}{q}{\lbl{l_i}\!:\! G'_i}{\lbl{i \in I}}}
	{l}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$\gtreduce{G_j}{G'_j}{l}$}
\AxiomC{$\subj{\lbl{l}} \neq \ppt{q}$}
\AxiomC{$\forall \lbl{i \in I \setminus \{ j \}} . ~ \gtype{G'_i} = \gtype{G_i}$}
\RightLabel{\rulename{Gr5}}
\TrinaryInfC{$
\gtreducelong
	{\gtrans{p}{q}{j}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}
	{\gtrans{p}{q}{j}{\lbl{l_i}\!:\! G'_i}{\lbl{i \in I}}}
	{l}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{}
\RightLabel{\colorbox{ColourShade}{\rulename{Gr6}}}
\UnaryInfC{$
\gtreducelong
	{\groute{p}{q}{s}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}
	{\gtransroute{p}{q}{s}{j}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}
	{\via{s}{\aout{p}{q}{j}}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{}
\RightLabel{\colorbox{ColourShade}{\rulename{Gr7}}}
\UnaryInfC{$
\gtreducelong
	{\gtransroute{p}{q}{s}{j}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}
	{\gtype{G_j}}
	{\via{s}{\ain{p}{q}{j}}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$\forall \lbl{i \in I}. ~ \gtreduce{G_i}{G'_i}{l}$}
\AxiomC{$\subj{\lbl{l}} \notin \{\ppt{p}, \ppt{q}\}$}
\RightLabel{\colorbox{ColourShade}{\rulename{Gr8}}}
\BinaryInfC{$
\gtreducelong
	{\groute{p}{q}{s}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}
	{\groute{p}{q}{s}{\lbl{l_i}\!:\! G'_i}{\lbl{i \in I}}}
	{l}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$\gtreduce{G_j}{G'_j}{l}$}
\AxiomC{$\subj{\lbl{l}} \neq \ppt{q}$}
\AxiomC{$\forall \lbl{i \in I \setminus \{ j \}} . ~ \gtype{G'_i} = \gtype{G_i}$}
\RightLabel{\colorbox{ColourShade}{\rulename{Gr9}}}
\TrinaryInfC{$
\gtreducelong
	{\gtransroute{p}{q}{s}{j}{\lbl{l_i}\!:\! G_i}{\lbl{i \in I}}}
	{\gtransroute{p}{q}{s}{j}{\lbl{l_i}\!:\! G'_i}{\lbl{i \in I}}}
	{l}
$}
\end{prooftree}

\captionof{figure}{LTS over Global Types in \newtheory}
\label{fig:newglobal}
\end{figure}

\begin{itemize}

\item \rulename{Gr6} and \rulename{Gr7}
are analogue to \rulename{Gr1} and \rulename{Gr2}
for describing the emission and reception of
messages in routed communication, but uses
the ``routed in-transit'' construct instead.

\item \rulename{Gr8} and \rulename{Gr9}
are analogue to \rulename{Gr4} and \rulename{Gr5}
in the sense that we only enforce the
syntactic order of messages for the participants
involved in the action $\lbl{l}$.

\end{itemize}

An important observation from
\rulename{Gr8} and \rulename{Gr9} is that,
for the router,
the syntactic order of routed communication
can be freely interleaved between
the syntactic order of direct communication.
This is a crucial result for proving
that the router does not over-serialise
communication.

\paragraph{LTS Semantics over Local Types}
We define the LTS semantics
over local types,
denoted by $\ltreduce{T}{T'}{l}$,
in \cref{fig:newlocal}.
We highlight and explain the new rules.

\begin{figure}[!h]

\begin{prooftree}
\AxiomC{}
\RightLabel{\rulename{Lr1}}
\UnaryInfC{$
\ltreducelong
	{\tsel{q}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{\ltype{T_j}}
	{\aout{p}{q}{j}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{}
\RightLabel{\rulename{Lr2}}
\UnaryInfC{$
\ltreducelong
	{\tbra{q}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{T_j}
	{\ain{q}{p}{j}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$
\ltreduce
	{T[\trec{T} / \trecvar]}
	{T'}
	{l}
$}
\RightLabel{\rulename{Lr3}}
\UnaryInfC{$
\ltreduce
	{\trec{T}}
	{T'}
	{l}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{}
\RightLabel{\colorbox{ColourShade}{\rulename{Lr4}}}
\UnaryInfC{$
\ltreducelong
	{\tselproxy{q}{s}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{T_j}
	{\via{s}{\aout{p}{q}{j}}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{}
\RightLabel{\colorbox{ColourShade}{\rulename{Lr5}}}
\UnaryInfC{$
\ltreducelong
	{\tbraproxy{q}{s}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{T_j}
	{\via{s}{\ain{q}{p}{j}}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{}
\RightLabel{\colorbox{ColourShade}{\rulename{Lr6}}}
\UnaryInfC{$
\ltreducelong
	{\router{p}{q}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{\routertrans{p}{q}{j}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{\via{s}{\aout{p}{q}{j}}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{}
\RightLabel{\colorbox{ColourShade}{\rulename{Lr7}}}
\UnaryInfC{$
\ltreducelong
	{\routertrans{p}{q}{j}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{T_j}
	{\via{s}{\ain{p}{q}{j}}}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$\forall \lbl{i \in I}. ~ \ltreduce{T_i}{T'_i}{l}$}
\AxiomC{$\subj{\lbl{l}} \notin \{\ppt{p}, \ppt{q}\}$}
\RightLabel{\colorbox{ColourShade}{\rulename{Lr8}}}
\BinaryInfC{$
\ltreducelong
	{\router{p}{q}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{\router{p}{q}{\lbl{l_i}\!:\! T'_i}{\lbl{i \in I}}}
	{l}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$\ltreduce{T_j}{T'_j}{l}$}
\AxiomC{$\subj{\lbl{l}} \neq \ppt{q}$}
\AxiomC{$\forall \lbl{i \in I \setminus \{ j \}}. ~ \ltype{T'_i} = \ltype{T_i}$}
\RightLabel{\colorbox{ColourShade}{\rulename{Lr9}}}
\TrinaryInfC{$
\ltreducelong
	{\routertrans{p}{q}{j}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{\routertrans{p}{q}{j}{\lbl{l_i}\!:\! T'_i}{\lbl{i \in I}}}
	{l}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$\lbl{l} = \lbl{\via{s}{\cdot}}$}
\AxiomC{$\subj{\lbl{l}} \neq \ppt{q}$}
\AxiomC{$\forall \lbl{i \in I}. ~ \ltreduce{T_i}{T'_i}{l}$}
\RightLabel{\colorbox{ColourShade}{\rulename{Lr10}}}
\TrinaryInfC{$
\ltreducelong
	{\tsel{q}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{\tsel{q}{\lbl{l_i}\!:\! T'_i}{\lbl{i \in I}}}
	{l}
$}
\end{prooftree}

\begin{prooftree}
\AxiomC{$\lbl{l} = \lbl{\via{s}{\cdot}}$}
\AxiomC{$\subj{\lbl{l}} \neq \ppt{q}$}
\AxiomC{$\forall \lbl{i \in I}. ~ \ltreduce{T_i}{T'_i}{l}$}
\RightLabel{\colorbox{ColourShade}{\rulename{Lr11}}}
\TrinaryInfC{$
\ltreducelong
	{\tbra{q}{\lbl{l_i}\!:\! T_i}{\lbl{i \in I}}}
	{\tbra{q}{\lbl{l_i}\!:\! T'_i}{\lbl{i \in I}}}
	{l}
$}
\end{prooftree}

\captionof{figure}{LTS over Local Types in \newtheory}
\label{fig:newlocal}
\end{figure}

We walk through rules \rulename{Lr4} and \rulename{Lr5}
from the perspective of role $\ppt{p}$.

\begin{itemize}

\item \rulename{Lr4} and \rulename{Lr5} are
analogue to \rulename{Lr1} and \rulename{Lr2}
for sending and receiving messages respectively.
The exception is that the new rules pattern-match
on the router role $\ppt{s}$ on the local type
and the routed label.

\end{itemize}

We walk through rules \rulename{Lr6}, \rulename{Lr7},
\rulename{Lr10} and \rulename{Lr11}
from the perspective of role $\ppt{s}$.

\begin{itemize}

\item \rulename{Lr6} and \rulename{Lr7} are
analogue to \rulename{Gr1} and \rulename{Gr2}.
Intuitively, the router $\ppt{s}$ holds a
``global'' perspective on the interaction
between $\ppt{p}$ and $\ppt{q}$, which explains
the correspondence with the LTS semantics over global
types.

\item \rulename{Lr10} and \rulename{Lr11} allow
the router to perform routing actions before handling
their own direct communication.
The syntax $\lbl{l} = \lbl{\via{s}{\cdot}}$
means that the label $\lbl{l}$ is ``of the form'' of a routing
action, i.e. there exists some $\ppt{p}, \ppt{q}, \lbl{j}$
such that $\lbl{l} = \lbl{\via{s}{\aout{p}{q}{j}}}$ or
$\lbl{l} = \lbl{\via{s}{\ain{p}{q}{j}}}$.
The constraint of $\subj{\lbl{l}} \neq \ppt{q}$
prevents the violation of the syntactic order of messages
sent and received by $\ppt{q}$.

Curious readers can consider the examples
$\proj{G_1}{s}$ and $\proj{G_2}{s}$
to see why this constraint is needed.

\begin{align*}
\gtype{G_1} &=
	\gcommone{s}{r}{\lbl{M1}}.~
	\grouteone{r}{q}{s}{\lbl{M2}}.~ \gtend \\
\proj{G_1}{s} &=
	\tselone{r}{\lbl{M1}}. ~
	\routerone{r}{q}{\lbl{M2}}{\gtend} \\
\gtype{G_2} &=
	\gcommone{s}{r}{\lbl{M1}}.~
	\grouteone{p}{r}{s}{\lbl{M2}}.~ \gtend \\
\proj{G_2}{s} &=
	\tselone{r}{\lbl{M1}}. ~
	\routerone{p}{r}{\lbl{M2}}{\gtend} \\
\end{align*}

\end{itemize}

As for the remaining rules,
\rulename{Lr8} and \rulename{Lr9} are analogue to
\rulename{Gr4} and \rulename{Gr5} because the router
holds a ``global'' perspective on the communication,
so transitions that do not violate the syntactic order
of messages between roles $\ppt{p}$ and $\ppt{q}$
are allowed.

